LPT: Less-overfitting Prompt Tuning for Vision-Language Model

Vision-language models (VLMs) have demonstrated exceptional generalization capabilities for downstream tasks. Due to its efficiency, prompt learning has gradually become a more effective and efficient method for transferring VLMs to downstream tasks, surpassing traditional finetuning methods. However, during the transfer process, these models are prone to severe overfitting, leading to a significant decline in generalization ability. To address this issue, we propose a framework named LPT, specifically designed for vision-language models. Specifically, we use CLIP to filter out fine-grained foreground information that may lead to overfitting, thereby guiding the prompts with basic visual concepts. Additionally, to further mitigate overfitting, we have developed a Structural Preservation (SP) constraint at the feature level, which aligns the model's overall feature space structure with the frozen CLIP, endowing the feature space with overall plasticity and enabling effective reshaping of the feature space during optimization. Moreover, we employ Hierarchical Logit (HL) constraint at the output layer to constrain the overall class information in the output, complementing the role of SP at the output end. Extensive experiments across various benchmarks (from base-to-novel, cross-dataset transfer, and domain generalization) demonstrate that our approach significantly improves generalization capability and effectively alleviates overfitting compared to state-of-the-art methods.

==> addon.tex <==
\newcommand{\argmax}{\mathop{\mathrm{arg max}}}
\newcommand{\argmin}{\mathop{\mathrm{arg min}}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\hf}{{\hat{f}}}
\newcommand{\p}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\frac{d #1}{d #2}}
\newcommand{\tP}{{\tilde{P}}}
\newcommand{\tf}{{\tilde{f}}}
\newcommand{\tp}{{\tilde{p}}}
\newcommand{\va}{{\bf a}}
\newcommand{\vb}{{\bf b}}
\newcommand{\vc}{{\bf c}}
\newcommand{\vd}{{\bf d}}
\newcommand{\ve}{{\bf e}}
\newcommand{\vf}{{\bf f}}
\newcommand{\vg}{{\bf g}}
\newcommand{\vl}{{\bf l}}
\newcommand{\vm}{{\bf m}}
\newcommand{\vh}{{\bf h}}
\newcommand{\vp}{{\bf p}}
\newcommand{\vq}{{\bf q}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vu}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\vvs}{{\bf s}}
\newcommand{\vt}{{\bf t}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\vz}{{\bf z}}
\newcommand{\vA}{{\bf A}}
\newcommand{\vB}{{\bf B}}
\newcommand{\vC}{{\bf C}}
\newcommand{\vD}{{\bf D}}
\newcommand{\vE}{{\bf E}}
\newcommand{\vF}{{\bf F}}
\newcommand{\vH}{{\bf H}}
\newcommand{\vG}{{\bf G}}
\newcommand{\vI}{{\bf I}}
\newcommand{\vM}{{\bf M}}
\newcommand{\vL}{{\bf L}}
\newcommand{\vO}{{\bf O}}
\newcommand{\vP}{{\bf P}}
\newcommand{\vQ}{{\bf Q}}
\newcommand{\vR}{{\bf R}}
\newcommand{\vW}{{\bf W}}
\newcommand{\vV}{{\bf V}}
\newcommand{\vS}{{\bf S}}
\newcommand{\vT}{{\bf T}}
\newcommand{\vX}{{\bf X}}
\newcommand{\vY}{{\bf Y}}
\newcommand{\vZ}{{\bf Z}}
\newcommand{\vK}{{\bf K}}
\newcommand{\vTheta}{{\bf \Theta}}
\newcommand{\vone}{{\bf 1}}
\newcommand{\vzero}{{\bf 0}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\lefteq}[1][2em]{\hspace{#1}&\hspace{-#1}}
\newcommand{\vmu}{{\boldsymbol \mu}}
\newcommand{\vtau}{{\boldsymbol \tau}}
\newcommand{\vSigma}{{\boldsymbol \Sigma}}
\newcommand{\vsigma}{{\boldsymbol \sigma}}
\newcommand{\vGamma}{{\boldsymbol \Gamma}}
\newcommand{\vgamma}{{\boldsymbol \gamma}}
\newcommand{\valpha}{{\bf \alpha}}
\newcommand{\tr}[1]{\mathrm{tr}\left(#1\right)}
\newcommand{\etr}[1]{\mathrm{etr}\left(#1\right)}
\newcommand{\vecz}[1]{\mathrm{vec}\left(#1\right)}
\newcommand{\trans}[1]{#1^\top}
\newcommand{\transinv}[1]{#1^{-\top}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\def\onedot{. }
% \def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
% \def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\st{s.t\onedot}
\def\dof{d.o.f\onedot}
\def\wrt{w.r.t\onedot}
\def\etal{\emph{et al}\onedot}


==> alg1.tex <==
\begin{algorithm}[t!]
\caption{Training phase of LPT}
\label{alg:train}
\setstretch{1.1}
\begin{algorithmic}[1]
\REQUIRE Training dataset $D_{train}=\{\mathbf{X},\mathbf{Y}\}$, where $\mathbf{X}=\{\boldsymbol{x}\}$ and $\mathbf{Y}=\{\boldsymbol{y}_{i}\}_{i=1}^{{N}}$; Text description $\mathbf{T}=\{\boldsymbol{t}_{i}\}_{i=1}^{{N}}$\\
\REQUIRE CLIP visual encoder \(f(\theta_f)\), text encoder \(g(\theta_g)\).

\STATE Obtain the attention mask of the input image \( \boldsymbol{x} \) using \(f(\theta_f)\).

\STATE Based on section \ref{sec:fim} and Eq. \ref{eq:mask}, use the mask to obtain the image ${\boldsymbol{x}^{'}}$ with the foreground information removed.

\STATE For the input image \( \boldsymbol{x}^{'} \) and input text \( \boldsymbol{t}_{i} \), add the vision prompt and text prompt respectively to obtain \( \tilde{\boldsymbol{x}} \) and \( \tilde{\boldsymbol{t}} \).

\STATE Obtain image features with prompt and text features with prompt: $\tilde{\boldsymbol{z}}$ $\gets$ $f(\tilde{\boldsymbol{x}}, \theta_f)$, $\tilde{\boldsymbol{v}}$$\gets$ $g(\tilde{\boldsymbol{t}}, \theta_g)$.

\STATE Obtain the visual and text features without any prompts: 
${\boldsymbol{z}}$ $\gets$ $f(\mathbf{x}, \theta_f)$, ${\boldsymbol{v}}$$\gets$ $g(\mathbf{t}, \theta_g)$.

\STATE Mix visual features from different layers through Eq.~\ref{eq:mix}:
${\tilde{\boldsymbol{z}}_{w}}$ $ \gets$ $\sum\limits_{i=1}^{H}{{{w}_{i}} \cdot {\tilde{\boldsymbol{z}}_{i}}}$; ${{\boldsymbol{z}}_{w}}$ $ \gets$ $\sum\limits_{i=1}^{H}{{{w}_{i}} \cdot {{\boldsymbol{z}}_{i}}}$.

\STATE Compute the logits ${\boldsymbol{p}}$ obtained from the frozen CLIP by Eq.~\ref{eq:zs_clip}.

\STATE Compute the logits $\tilde{\boldsymbol{p}}$ after adding the prompt by Eq.~\ref{eq:pmt_clip}.

\STATE  Compute the cross-entropy loss through Eq.~\ref{eq:ce}.

\STATE Compute the local angular relationship $\boldsymbol{A}$ of the image features obtained from the frozen CLIP by Eq.~\ref{eq:zs_abgle}.

\STATE Compute the local angular relationship $\tilde{\boldsymbol{A}}$ of the image features obtained after adding the prompt by Eq.~\ref{eq:pmt_abgle}.

\STATE Compute the visual loss ${\mathcal{L}_{vision}}$ and text loss ${\mathcal{L}_{text}}$ using Eq.~\ref{eq:loss_vision} and Eq.~\ref{eq:loss_text}, respectively.

\STATE Compute the instance-aware constraint~${{\mathcal{L}}_{ia}}$ and class-aware constraint~${\mathcal{L}_{ca}}$ using Eq. \ref{eq:ia_loss} and Eq. \ref{eq:ca_loss}, respectively.
\end{algorithmic}
\end{algorithm}
\vspace{-7mm}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/Method.tex <==

\section{Method}
\subsection{Preliminary}
% \textbf{Contrastive Language-Image}\textbf{ Pretraining(CLIP).} CLIP ~\cite{clip} consists of two sub-networks, referred to as the image encoder and the text encoder. By understanding image-text pairs, CLIP constructs a shared embedding space \(\mathbb{R}^{\rm{d}}\), where \(\rm{d}\) denotes the feature embedding dimension. The image encoder and text encoder of CLIP are denoted as \(f({\theta_f})\) and \(g({\theta_g})\), where \({\theta_f}\) and \({\theta_g}\) represent the parameters of \(f\) and \(g\). Given an image \(x\) and class labels \(\boldsymbol{\rm{Y}} = \{\boldsymbol{y}_{1}, \boldsymbol{y}_{2}, \ldots, \boldsymbol{y}_{i}, \ldots, \boldsymbol{y}_{{N}} \}\) (\({\rm{N}}\) is the number of classes), the image encoder generates the corresponding image feature \(\boldsymbol{z} = f(\boldsymbol{x}, \theta_f) \in \mathbb{R}^\rm{d}\). The text encoder then generates the corresponding text features \(\boldsymbol{\rm{V}} = \{ {\boldsymbol{v}_{i}}=g(\boldsymbol{t}_i, \theta_g) \in \mathbb{R}^d \}_{i=1}^{{N}}\) using handcrafted text templates \(\boldsymbol{t}_i = \text{``a photo of [CLASSNAME}_i\text{]}"\).
\noindent\textbf{Contrastive Language-Image Pretraining (CLIP).} CLIP~\cite{clip} consists of two sub-networks, referred to as the image encoder and the text encoder. By understanding image-text pairs, CLIP constructs a shared embedding space \(\mathbb{R}^{d}\), where \(d\) denotes the feature embedding dimension. The image encoder and text encoder of CLIP are denoted as \(f(\theta_f)\) and \(g(\theta_g)\), where \(\theta_f\) and \(\theta_g\) represent the parameters of \(f\) and \(g\). Given an image \(x\) and class labels \(\mathbf{Y} = \{{\boldsymbol{y}}_{1}, {\boldsymbol{y}}_{2}, \ldots, {\boldsymbol{y}}_{i}, \ldots, {\boldsymbol{y}}_{N} \}\) (\(N\) is the number of classes), the image encoder generates the corresponding image feature \(\mathbf{z} = f({\boldsymbol{x}}, \theta_f) \in \mathbb{R}^{d}\). The text encoder then generates the corresponding text features \(\mathbf{V} = \{ {\boldsymbol{v}}_{i} = g({\boldsymbol{t}}_i, \theta_g) \in \mathbb{R}^d \}_{i=1}^{N}\) using handcrafted text templates \({\boldsymbol{t}}_i = \text{``a photo of [CLASSNAME}_i\text{]''}\).

Finally, using cosine similarity, CLIP predicts the class for a given image \(x\):
\begin{equation}
\label{eq:zs_clip}
    \boldsymbol{p}({\boldsymbol{y}}=i|\boldsymbol{x})=\frac{\exp ({\rm{sim}}(\boldsymbol{z},{\boldsymbol{v}_{i}})/{\tau})}{\sum\nolimits_{j=1}^{{N}}{\exp ({\rm{sim}}(\boldsymbol{z},{\boldsymbol{v}_{j}})/{\tau})}},
\end{equation}
where, ${\rm{sim}}(\boldsymbol{z},{{\boldsymbol{v}_{j}})}=\frac{\boldsymbol{z} \cdot {\boldsymbol{v}_{j}}}{\|\boldsymbol{z}\| \times \|{\boldsymbol{v}_{j}}\|}$ denotes the cosine similarity, and ${\tau}$ is the temperature coefficient.

\noindent\textbf{Soft Prompt Tuning.}
Based on IVLP~\cite{IVLP}, we add learnable visual and text prompts to the image and text encoders, denoted as $\boldsymbol{P}_v = \{\boldsymbol{p}_v^i\}_{i=1}^K$ and $\boldsymbol{P}_l = \{\boldsymbol{p}_l^i\}_{i=1}^L$, respectively. Here, $K$ and $L$ represent the number of learnable tokens. Therefore, the inputs to the image and text encoders become: $\tilde{\boldsymbol{x}} = [\boldsymbol{P}_v, \boldsymbol{x}]$ and $\tilde{\boldsymbol{t}}_i = [\boldsymbol{P}_l, \boldsymbol{t}_i]$. The resulting image feature is $\tilde{\boldsymbol{z}} = f(\tilde{\boldsymbol{x}}, \theta_f) \in \mathbb{R}^d$, and the text features are $\tilde{\boldsymbol{V}} = \{{{{\tilde{\boldsymbol{v}}}}_{i}}=g(\tilde{\boldsymbol{t}}_i, \theta_g) \in \mathbb{R}^d\}_{i=1}^N$. Similarly, the prediction for a given image $x$ in CLIP is:
\begin{equation}
\label{eq:pmt_clip}
    \tilde{\boldsymbol{p}}({\boldsymbol{y}}=i|\boldsymbol{x})=\frac{\exp (\rm{sim}(\tilde{\boldsymbol{z}},{{{\tilde{\boldsymbol{v}}}}_{i}})/{\tau})}{\sum\nolimits_{j=1}^{{N}}{\exp (\rm{sim}(\tilde{\boldsymbol{z}},{{{\tilde{\boldsymbol{v}}}}_{j}})/{\tau})}}.
\end{equation}
\indent To further optimize the prompts and make them more suitable for the downstream dataset ${\mathcal{D}}$, Cross-Entropy loss is used for optimization, as follows:
\begin{equation}
\label{eq:ce}
    {{\mathcal{L}}_{cls}}=-\tfrac{1}{{{{N}}_{D}}}\sum\limits_{i=1}^{{{{N}}_{D}}}{({{\boldsymbol{y}}_{i}}\cdot \log ({{{\tilde{\boldsymbol{p}}}}_{i}})}),
\end{equation}
where, \({{{N}}_{D}}\) is the number of exemplars in the downstream dataset ${\mathcal{D}}$, and \({{\boldsymbol{y}}_{i}}\) and \({{\tilde{\boldsymbol{p}}}_{i}}\) are the true label and the predicted value for the downstream data \({{\boldsymbol{x}}_{i}}\), respectively.
%-----------------------------------------------------
% \subsection{An Insight into Generalization Decline in Base-to-Novel}
% %\subsection{An Insight into Overfitting Problem in Base-to-Novel}
% In Base-to-Novel tasks, due to the invisibility of novel class data, the better the generalization performance on the base (or target) task, the worse it tends to be on novel tasks, and vice versa. For instance, in the case of CoOp~\cite{coop}, the introduction of prompts facilitates the model's fitting of fine-grained features of base classes during the few-shot stage, enhancing its learning capability with a small number of samples. However, this fitting of base class details poses challenges to zero-shot generalization, creating a contradictory relationship between the two.

% As shown in Figure 1, the model's excessive focus on base class data leads to an over-reliance on specific features. This over-reliance causes overfitting, which is the root cause of the decline in generalization capability to novel classes in base-to-novel tasks. From an informational perspective, overfitting causes the model to overly focus on fine-grained foreground information of the base classes (Figure \ref{fig:head}), resulting in diffuse attention on novel class data and an inability to accurately capture new class information. Furthermore, overfitting can steer the model's feature space towards a suboptimal direction, hindering the transfer of learned knowledge to unseen classes.

% Therefore, we address the overfitting issue in base-to-novel tasks from two perspectives: information selection and feature space optimization.
%------------------------------------------------------
\begin{figure}[t!]
\begin{center}
\centerline{\includegraphics[width=0.9\linewidth]{fig/mask.pdf}}
\caption{Details of the Foreground Information Mask (FIM). This figure illustrates the FIM process in our method. Through FIM, the high-attention regions of the image are filtered out, retaining only the fundamental visual information of the image (e.g., pose, fur color, etc.).}

\label{fig:mask}
\end{center}
\vspace{-3mm}
\end{figure}

\subsection{Foreground Information Mask}
\label{sec:fim}
VLMs are transferred to downstream tasks through prompt tuning, which enhances the model's focus on fine-grained foreground information within the training data, facilitating effective transfer. However, in B2N tasks involving unseen downstream challenges, prompt tuning can cause the model to overly fit the training data, leading to the neglect of essential underlying visual information and ultimately degrading performance on unseen data.

To address the overfitting issue mentioned above, we propose a mask mechanism to reduce excessive attention to local information. We use the attention map of each training image to capture its foreground information and construct a mask to filter part of them. Specifically, we apply a threshold to the attention maps: attention blocks with values greater than the threshold are set to 0, while the rest are set to 1, to create a mask. 

Then, we use the obtained mask to filter the foreground fine-grained information of the image:
\begin{equation}
\label{eq:mask}
    {\boldsymbol{x}^{'}}={\rm{mask}}\odot{ \boldsymbol{x}},
\end{equation}
\noindent where the $\odot$ denotes element-wise multiplication. By using a mask, we can filter out the parts of the input image that are most likely to cause overfitting. This forces the model to focus more on the underlying visual information when transferring to downstream tasks. This approach helps improve the model's ability to generalize to unknown data in downstream tasks.


%------------------------------------------------------
\subsection{Structural Preservation Constraint}
We leverage an exemplar relationship graph to mine CLIP's zero-shot knowledge and use angle-based feature structural preservation to impart a degree of flexibility to CLIP's original feature space, thereby enabling holistic transfer to downstream tasks. By retaining \textbf{angular relationships between samples} instead of point-to-point constraints, we preserve the topological structure of the original CLIP. This maintains CLIP’s generalization ability without limiting prompt adaptability to downstream tasks.

Given any three samples ${{x}_{i}},{{x}_{j}},{{x}_{k}}$ in the feature topology space, they form a local angular relationship $\boldsymbol{A}$, where $\boldsymbol{A}$ is used for the frozen CLIP, and $\tilde{\boldsymbol{A}}$ is used for the model after prompt tuning.

Due to the different semantic information contained in various layers of ViT, we perform weighted combinations of features from different ViT layers to further supplement the lost low-level visual information during the model fitting process. The fused image feature is obtained as follows:
\begin{equation}
\label{eq:mix}
    {{\boldsymbol{z}}_{w}}=\sum\limits_{i=1}^{H}{{{w}_{i}} \cdot {{\boldsymbol{z}}_{i}}},
\end{equation}
where \({{\boldsymbol{z}}_{i}}\) is the feature from the \(i\)-th ViT layer of the image encoder, $H$ is the number of ViT layers, and \({{w}_{i}}\) is the weight obtained through Gaussian sampling, with \(\sum\limits_{i}{{w}_{i}}=1\).
Therefore, for the frozen CLIP model, the local angular relationship \(\boldsymbol{A}\) of samples \({{x}_{i}}, {{x}_{j}}, {{x}_{k}}\) is expressed as:
\begin{equation}
\label{eq:zs_abgle}
  {\boldsymbol{A}}\left( {{x}_{i}},{{x}_{j}},{{x}_{k}} \right) = \frac{{{\boldsymbol{e}}_{ij}} \cdot {{\boldsymbol{e}}_{kj}}}{\left\| {{\boldsymbol{e}}_{ij}} \right\| \left\| {{\boldsymbol{e}}_{kj}} \right\|}  ,
\end{equation}
where ${{\boldsymbol{e}}_{ij}} = {{\boldsymbol{z}}_{w,i}} - {{\boldsymbol{z}}_{w,j}}$ and ${{\boldsymbol{e}}_{kj}} = {{\boldsymbol{z}}_{w,k}} - {{\boldsymbol{z}}_{w,j}}$ represent the distance vectors between two samples in the feature space.

Similarly, for the model after prompt tuning, the local angular relationship \(\tilde{A}\) of samples \({{x}_{i}}, {{x}_{j}}, {{x}_{k}}\) is expressed as:
\begin{equation}
\label{eq:pmt_abgle}
\tilde{\boldsymbol{A}}\left({{x}_{i}},{{x}_{j}},{{x}_{k}} \right) = \frac{{{{\tilde{\boldsymbol{e}}}}_{ij}} \cdot {{{\tilde{\boldsymbol{e}}}}_{kj}}}{\left\| {{{\tilde{\boldsymbol{e}}}}_{ij}} \right\| \left\| {{{\tilde{\boldsymbol{e}}}}_{kj}} \right\|},
\end{equation}
where \({{{\tilde{\boldsymbol{e}}}}_{ij}} = {{\tilde{\boldsymbol{z}}}_{w,i}} - {{{\tilde{\boldsymbol{z}}}}_{w,j}}\) and \({{{\tilde{\boldsymbol{e}}}}_{kj}} = {{\tilde{\boldsymbol{z}}}_{w,k}} - {{\tilde{\boldsymbol{z}}}_{w,j}}\).
The local angular relationship function between samples reflects the angular structure of the feature topology space. We aim to maintain this structure during the CLIP's transfer to downstream tasks. Therefore, our structural preservation constraint is as follows:
\begin{equation}
\label{eq:loss_vision}
    {\mathcal{L}_{vision}}({{x}_{i}},{{x}_{j}},{{x}_{k}})={{\left\| \tilde{\boldsymbol{A}}-\boldsymbol{A} \right\|}_{1}}.
\end{equation}

Due to the sparse and relatively fixed nature of textual information, to maintain consistency in the text space, we use the L1 distance to constrain the text space for a given text $t$:
\begin{equation}
\label{eq:loss_text}
   {{\mathcal{L}}_{text}}={{\left\| g(\tilde{\boldsymbol{t}},{{\theta }_{g}})-g({\boldsymbol{t}},{{\theta }_{g}}) \right\|}_{1}},
\end{equation}
where the \( g({{\theta }_{g}}) \) is the text encoder, \( \tilde{t} \) is the text input with the prompt added, and \( t \) is the original text input.

Our SP does not directly constrain the movement of individual samples in the feature space. Instead, it constrains the change in feature space structure by maintaining angular relationships, allowing reasonable displacement of samples in the feature space during the optimization process. This soft constraint is easier to optimize and imparts a degree of plasticity to the feature space, making its structure flexible.

Overall, our SP loss is defined as follows:
\begin{equation}
    {{\mathcal{L}}_{\rm{SP}}}={{\mathcal{L}}_{vision}}+{{\mathcal{L}}_{text}}.
\end{equation}
\input{alg1}
%--------------------------------------------------------------
\subsection{Hierarchical Logit Constraint}
To further complement SP at the model output and inherit CLIP's knowledge of the relationships between different samples, we constrain the model output at different layers of the logits. We believe logits for a single example contain specific information, and distilling knowledge from them may alter the encompassing topological structure. Hence, we use hierarchical logit constraint for model consistency supplementation.

\noindent\textbf{Instance-aware Constraint.} Following the traditional knowledge distillation approach ~\cite{KD}, we use KL divergence to achieve alignment with the frozen CLIP space at the instance awareness as follows:
\begin{equation}
\label{eq:ia_loss}
\begin{split}
    {{\mathcal{L}}_{ia}} &={{\mathcal{D}_{KL}}}(\boldsymbol{p}({\boldsymbol{y}}|\boldsymbol{x}) \parallel \boldsymbol{\tilde{p}}(\boldsymbol{y}|\boldsymbol{x})) \\
     &=\sum_{i} \boldsymbol{p}({\boldsymbol{y}}=i|\boldsymbol{x}) \log \left(\frac{\boldsymbol{p}({\boldsymbol{y}}=i|\boldsymbol{x})}{\boldsymbol{\tilde{p}}({\boldsymbol{y}}=i|\boldsymbol{x})}\right),
\end{split}
\end{equation}
where, $\boldsymbol{p}$ represents the logits from the frozen CLIP, while $\boldsymbol{\tilde{p}}$ represents the logits from the prompt-tuned model. The loss function $ {{\mathcal{L}}_{ia}}$ aligns the model with the frozen CLIP at the instance awareness, providing fundamental spatial alignment.

%----------------------------------------------------------------------

%----------------------------------------------------------------------

\noindent\textbf{Class-aware Constraint.} We consider that the output of the prompt-tuned model and the output of the frozen CLIP model should exhibit similar distribution descriptions across classes. 

We denote \( M \) and \( \tilde{M} \) as the class relationship matrices for the frozen CLIP and the model after prompt tuning, respectively. Given the logits $\boldsymbol{p}$ of the frozen CLIP and the logits $\boldsymbol{\tilde{p}}$ of prompt-tuned model, they are computed as follows:

\begin{equation}
     M={\boldsymbol{p}^{T}}\cdot \boldsymbol{p}, \indent \tilde{M}={\boldsymbol{\tilde{p}}^{T}}\cdot \boldsymbol{\tilde{p}},
\end{equation}
where, \( M \) and \(\tilde{M}\) are \( C \times C \) matrices, where \( C \) is the number of classes. \( M_{ij} \) and \( \tilde{M}_{ij} \) represent the probabilities that a sample belongs simultaneously to class \( i \) and class \( j \).

Given the class relationship matrices, the following constraints apply:
\begin{equation}
\label{eq:ca_loss}
    {{\mathcal{L}_{ca}}=\frac{1}{C}{{\left\| M-\tilde{M} \right\|}_{2}}}.
\end{equation}

Through ${\mathcal{L}_{ca}}$, we further supplement the lost class information during the model transfer process, achieving model consistency at the class awareness.

Our hierarchical logit constraint is:
\begin{equation}
    {\mathcal{L}_{\rm{HL}}}={{\mathcal{L}}_{ia}}+{\mathcal{L}_{ca}}.
\end{equation}

Overall, our final loss function is as follows:
\begin{equation}
    \mathcal{L}={{\mathcal{L}_{cls}}+{\lambda }{\mathcal{L}_{\rm{HL}}}+{\gamma}{\mathcal{L}_{\rm{SP}}}},
\end{equation}
\noindent where, $\gamma$ and $\lambda$ are hyperparameters.
%----------------------------------------------------------------------

% \clearpage
\input{tables/b2n_main}

==> tables/b2n_main.tex <==
\begin{table*}[t!] 
\caption{Compare the performance on 4 challenging datasets, 7 easy datasets and all 11 datasets of our method with existing methods on base-to-novel generalization. For base-to-novel generalization, based on the performance of zero-shot CLIP, we classify DTD, FGVCAircraft, EuroSAT, and UCF101 as challenging datasets. These four datasets have fine-grained characteristics, making them more prone to overfitting compared to other datasets. The best results are in \textbf{bold} and the second-best results are \underline{underlined}. The model size used by all comparison methods is consistent.}
\centering
\renewcommand{\arraystretch}{0.92}
{\fontsize{9pt}{12pt}\selectfont

    \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{Average over 4 challenging datasets.}}
    \begin{tabular}{l cc|c}
    \toprule
    Method & Base & Novel & HM \\
    \midrule
    CLIP~\cite{clip} & 51.86 & 59.44 & 55.39 \\ 
    CoOp~\cite{coop} & 74.19 & 43.57 & 54.90 \\ 
    CoCoOp~\cite{cocoop} & 70.04 & 52.95  &	60.30  \\
    LASP~\cite{lasp} & 73.83 & 61.25 & 66.95  \\ 	
    MaPLe~\cite{maple} & 73.72 & 61.67 & 67.16 \\ 	 	 
    PromptSRC~\cite{promptsrc} & {76.53} & {63.39} & {69.34}  \\ 	 	 	
    Dept~\cite{dept} & 75.06 & 60.57 & 67.04 \\ 
    TCP~\cite{tcp} & 75.88 & 62.00 & 68.24 \\ 	
    MMA~\cite{mma} & 73.87 & \underline{66.08} & \underline{69.45} \\ 
    2SFS~\cite{2SFS} & \textbf{79.21} & 61.45 & 69.05 \\
    \midrule
    \textbf{LPT (Ours)}  & \underline{78.03} & \textbf{66.27} & \textbf{71.62} \\
    \bottomrule
    \end{tabular}
    \end{minipage}
    ~
    \begin{minipage}[t]{0.32\textwidth}
    \centering
     \caption*{\textbf{Average over 7 easy datasets.}}
    \begin{tabular}{l cc|c}
    \toprule
    Method & Base & Novel & HM \\
    \midrule
    CLIP~\cite{clip} & 79.33 & 82.67 & 80.96 \\ 	 
    CoOp~\cite{coop} & 87.55 & 74.45 & 80.47 \\
    CoCoOp~\cite{cocoop} & 86.43 & 82.40 & {84.37} \\
    LASP~\cite{lasp} & 87.77 & 82.70 & 85.16 \\ 	 	 
    MaPLe~\cite{maple} & 87.17 & 82.84 & 84.95 \\	 	 
    PromptSRC~\cite{promptsrc} & {88.68} &{83.37} & {86.05} \\  	 	 	
    Dept~\cite{dept} & 88.51 & 83.31 & 85.83  \\
    TCP~\cite{tcp} & {88.85} & 82.99 & 85.82 \\
    MMA~\cite{mma} & 88.54 & 83.14 & 85.59 \\ 
    2SFS~\cite{2SFS} & \textbf{89.18} & \underline{83.49} & \underline{86.07} \\
    \midrule 	
   \textbf{LPT (Ours)}  & \underline{89.14} & \textbf{84.06} & \textbf{86.40} \\
    \bottomrule 	 	
    \end{tabular}
    \end{minipage}
    ~
    \begin{minipage}[t]{0.32\textwidth}
    \centering 
   \caption*{\textbf{Average across all 11 datasets.}}
    \begin{tabular}{l cc|c}
    \toprule
    Method & Base & Novel & HM \\
    \midrule
    CLIP~\cite{clip} & 69.34 & 74.22 & 71.70 \\
    CoOp~\cite{coop} & 82.69 & 63.22 & 71.66 \\
    CoCoOp~\cite{cocoop} & 80.47 & 71.69 & 75.83 \\
    LASP~\cite{lasp} & 82.70 & 74.90 & 78.61 \\
    MaPLe~\cite{maple} & 82.28 & 75.14 & 78.55 \\
    PromptSRC~\cite{promptsrc} & {84.26} & {76.10} & {79.97} \\
    Dept~\cite{dept} & 83.62 & 75.04 & 79.10 \\
    TCP~\cite{tcp} & {84.13} & 75.36 & 79.51 \\
    MMA~\cite{mma} & 83.20  &  \underline{76.80} & 79.87 \\ 
    2SFS~\cite{2SFS} &  \textbf{85.55} & 75.48 &  \underline{80.20} \\
    \midrule 
   \textbf{LPT (Ours)}  &  \underline{85.10} & \textbf{77.59} & \textbf{81.02} \\
    \bottomrule
    \end{tabular}
    \end{minipage}
}

\label{tab:base2novel}
\end{table*}
